Pragmatic Neural Language Modelling in Machine Translation

This paper presents an in-depth investigation on integrating neural language models in translation systems. Scaling neural language models is a difficult task, but crucial for real-world applications. This paper evaluates the impact on end-to-end MT quality of both new and existing scaling techniques. We show when explicitly normalising neural models is necessary and what optimisation tricks one should use in such scenarios. We also focus on scalable training algorithms and investigate noise contrastive estimation and diagonal contexts as sources for further speed improvements. We explore the trade-offs between neural models and back-off n-gram models and find that neural models make strong candidates for natural language applications in memory constrained environments, yet still lag behind traditional models in raw translation quality. We conclude with a set of recommendations one should follow to build a scalable neural language model for MT.

==> Background.tex <==
\section{Background}

Language models are used in translation systems to improve the fluency of the output translations. In most systems, the default language model implementation is a back-off n-gram language model with Kneser-Ney smoothing \citep{Chen1999}. Back-off n-gram models are conceptually simple, very efficient to construct and query, and are regarded as being extremely effective in translation systems.

Neural language models are a more recent class of language models \citep{Bengio2003} that have been shown to outperform back-off n-gram models using intrinsic evaluation \citep{Chelba2013, Bengio2003} or as part of other natural language systems such as speech recognizers \citep{Mikolov2011, Schwenk2007}. Neural language models effectively combat the problem of data sparsity inherent to standard n-gram models by learning distributed representations for words in a continuous vector space. The language modelling probabilities are estimated by projecting a word's context in the same space as the word representations and by assigning probabilities proportional to the distance between the words and the context's projection. This procedure effectively assigns a non-zero probability to every word in the vocabulary. 


